Be Intentional About Fairness!: Fairness, Size, and Multiplicity in the Rashomon Set

When selecting a model from a set of equally performant models, how much unfairness can you really reduce? Is it important to be intentional about fairness when choosing among this set, or is arbitrarily choosing among the set of ''good'' models good enough? Recent work has highlighted that the phenomenon of model multiplicity-where multiple models with nearly identical predictive accuracy exist for the same task-has both positive and negative implications for fairness, from strengthening the enforcement of civil rights law in AI systems to showcasing arbitrariness in AI decision-making. Despite the enormous implications of model multiplicity, there is little work that explores the properties of sets of equally accurate models, or Rashomon sets, in general. In this paper, we present five main theoretical and methodological contributions which help us to understand the relatively unexplored properties of the Rashomon set, in particular with regards to fairness. Our contributions include methods for efficiently sampling models from this set and techniques for identifying the fairest models according to key fairness metrics such as statistical parity. We also derive the probability that an individual's prediction will be flipped within the Rashomon set, as well as expressions for the set's size and the distribution of error tolerance used across models. These results lead to policy-relevant takeaways, such as the importance of intentionally looking for fair models within the Rashomon set, and understanding which individuals or groups may be more susceptible to arbitrary decisions.

==> takeaway1avg_vs_opt.tex <==
\section{The Importance of Intentional Fairness}\label{sec:intentional}

\begin{figure}[htp]
    \centering
    % First subfigure
    \begin{subfigure}[b]{0.32\textwidth}  % Adjust width to your needs
        \centering
        \includegraphics[width=\textwidth]{facct_submission/figures/PPR_disparity_german_1-13-2025.png}  % Replace with your image
    \end{subfigure}
    \hfill
    % Second subfigure
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{facct_submission/figures/PPR_disparity_adult_1-13-2025.png}  % Replace with your image
    \end{subfigure}
     % Second subfigure
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{facct_submission/figures/PPR_disparity_health_1-13-2025.png}  % Replace with your image
    \end{subfigure}
    \caption{Disparity in positive prediction rate for the German, Adult, and Health datasets, as a function of the error tolerance $\epsilon$. Comparison of methods for optimizing PPR (Section~\ref{sec:optimizing-PPR}), uniform random sampling (Section~\ref{sec:sampling}), and sampling linear models (Section~\ref{sec:linear}) over the Rashomon set $R_N(\epsilon)$.}
    \label{fig:PPR_disparity}
\end{figure}

\begin{figure}[htp]
    \centering
    % First subfigure
    \begin{subfigure}[b]{0.32\textwidth}  % Adjust width to your needs
        \centering
        \includegraphics[width=\textwidth]{facct_submission/figures/FPR_disparity_german_1-13-2025.png}  % Replace with your image
    \end{subfigure}
    \hfill
    % Second subfigure
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{facct_submission/figures/FPR_disparity_adult_1-13-2025.png}  % Replace with your image
    \end{subfigure}
     % Second subfigure
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{facct_submission/figures/FPR_disparity_health_1-13-2025.png}  % Replace with your image
    \end{subfigure}
    \caption{Disparity in false positive rate for the German, Adult, and Health datasets, as a function of the error tolerance $\epsilon$. Comparison of methods for optimizing FPR (Section~\ref{sec:optimizing-TPR and FPR}), uniform random sampling (Section~\ref{sec:sampling}), and sampling linear models (Section~\ref{sec:linear}) over the Rashomon set $R_N(\epsilon)$.}
    \label{fig:FPR_disparity}
\end{figure}

\begin{figure}[htp]
    \centering
    % First subfigure
    \begin{subfigure}[b]{0.32\textwidth}  % Adjust width to your needs
        \centering
        \includegraphics[width=\textwidth]{facct_submission/figures/TPR_disparity_german_1-13-2025.png}  % Replace with your image
    \end{subfigure}
    \hfill
    % Second subfigure
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{facct_submission/figures/TPR_disparity_adult_1-13-2025.png}  % Replace with your image
    \end{subfigure}
     % Second subfigure
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{facct_submission/figures/TPR_disparity_health_1-13-2025.png}  % Replace with your image
    \end{subfigure}
    \caption{Disparity in true positive rate for the German, Adult, and Health datasets, as a function of the error tolerance $\epsilon$. Comparison of methods for optimizing TPR (Section~\ref{sec:optimizing-TPR and FPR}), uniform random sampling (Section~\ref{sec:sampling}), and sampling linear models (Section~\ref{sec:linear}) over the Rashomon set $R_N(\epsilon)$.}
    \label{fig:TPR_disparity}
\end{figure}

%In this Section, we demonstrate the importance of explicitly searching for fair models within the Rashomon set. 

A natural question that may come up when considering searching for fairer models within the Rashomon set is---is it worth it? What if the fairness of all the models in the Rashomon set is more or less the same, and a randomly sampled model---akin to selecting a model solely on the basis of accuracy and not paying attention to fairness---is just as fair as the fairest ones within the set?
In this Section, we show that this is definitely not the case--- the fairness difference between the average, or randomly sampled, model within the Rashomon set and the fairest models can be very large. We also show experimentally that how you look for fairer models can influence your success---while searching directly for the fairest model via our algorithm is always the most effective method, whether you can reach significantly fairer models by randomly sampling models in the Rashomon set is dataset dependent, and also depends on how you search.

To compare what we gain by being intentional or arbitrary about fairness within the Rashomon set, 
we must show both how to draw randomly from the Rashomon set and how to find the fairest model.
We present \textbf{novel, computationally efficient approaches} for (i) optimizing different fairness metrics over the Rashomon set, as described in Section~\ref{sec:optimizing-fairness}; and (ii) sampling models uniformly at random from the Rashomon set, as described in Section~\ref{sec:sampling}.  We also describe a simple baseline for comparison in Section~\ref{sec:linear}: restricting the model class (here we assume penalized logistic regression models) and learning models from that class with different sources of random variation.  We compare the fairness of the models found by the optimization, uniform sampling, and restricted model class approaches in Section~\ref{sec:intentional-experiments}, and explore policy takeaways in Section~\ref{sec:intentional-takeaways}. 

\subsection{Optimizing fairness over the Rashomon set}
\label{sec:optimizing-fairness}

Despite computational hardness results for finding the fairest model in the Rashomon set~\cite{laufer2024fundamental}, we show that under certain conditions, it is possible to find the fairest model within the Rashomon set $R_N(\epsilon)$ defined on $N$ data records in log-linear time, $\mathcal{O}(N \log N)$. In particular, when we are concerned with mitigating demographic disparity (i.e., equalizing the positive prediction rate or PPR) between two groups, we show that we can find the exact fairest model within the Rashomon set. For equalizing false positive rate (FPR) or true positive rate (TPR) between two groups, we can find a model which is guaranteed to have error rate disparity no more than $\mathcal{O}(\frac{1}{N})$ higher than the fairest model. As we show below, using these algorithms on three real-world datasets, we see that in practice, it is often possible to completely eradicate disparities by searching within the Rashomon set for very small $\epsilon$--- less than half of a percent in many cases.

For PPR, FPR, and TPR, we can express the optimization of the fairness criterion over flip vectors $\theta$, subject to the constraint that 
$\theta$ is in the Rashomon set $R_N(\epsilon)$, as a \emph{knapsack problem}, where each data record $d_i$ has a weight $w_i = |2p_i-1|$ and a value $v_i$ defined below, and $\theta_i=1$ corresponds to the inclusion of element $i$ in the knapsack, adding $w_i$ to the total weight and $v_i$ to the total value.  The 0-1 knapsack problem is then the constrained optimization with capacity $N\epsilon$: $\max \sum_i \theta_i v_i$ subject to $\theta_i \in \{0,1\}$ and $\sum_i \theta_i w_i \le N\epsilon$. While this problem is NP-hard to solve in general, we present efficient solutions for the special cases below.

\dn{To do: compare complexity of our solution to Laufer et al. Previous sentence was: Laufer et al.~\cite{laufer2024fundamental} present a more general approximation algorithm which requires exponential time (CHECK THIS!)-- so while their algorithm works in more circumstances (e.g., for more than two groups), ours is much faster when it applies.}  
 
\subsubsection{Optimizing for statistical parity}
\label{sec:optimizing-PPR}
Let $P_A$ and $P_B$ be the vectors of Bayes-optimal probabilities $p_i$ for subgroups $A$ (the \emph{protected class}, data records $d_i$ with sensitive attribute value $A_i=a$) and $B$ (the \emph{non-protected class}, data records $d_i$ with sensitive attribute value $A_i\ne a$) respectively. Let $F^\text{opt} = \langle F_A^\text{opt}, F_B^\text{opt} \rangle$ denote the vector of Bayes-optimal binary predictions $f_\text{opt}(x_i)$, and let $F = \langle F_A,F_B\rangle$ denote the vector of binary predictions $f(x_i)$ corresponding to flip vector $\theta = \langle \theta_A, \theta_B\rangle$.  \ignore{We note that
$F_N = F_N^\text{opt} \odot (1 - \theta) + (1 - F_N^\text{opt}) \odot \theta$,
where $\odot$ is the element-wise product between two vectors.}  As shown in Appendix~\ref{appendix:statdisp}, we define the positive prediction rate disparity as: 
\begin{align*}
\text{disparity}_{PPR} = \left|\mathbf{E}[f(x_i) \:|\: d_i\in A] - \mathbf{E}[f(x_i) \:|\: d_i \in B] \right| = \left|\frac{||F_A||_1}{|A|} - \frac{||F_B||_1}{|B|}\right|,
\end{align*}
where $F_A = F^\text{opt}_A \odot (1-\theta_A) + (1-F^\text{opt}_A) \odot \theta_A$, $F_B = F^\text{opt}_B \odot (1-\theta_B) + (1-F^\text{opt}_B) \odot \theta_B$, and $\odot$ denotes element-wise product. Assume wlog that subgroup $A$ has higher PPR, $\frac{||F_A||_1}{|A|} > \frac{||F_B||_1}{|B|}$. Then flipping a prediction in group $A$ from 1 to 0, or flipping a prediction in group $B$ from 0 to 1, reduces disparity by $\frac{1}{|A|}$ or $\frac{1}{|B|}$ respectively, while other flips increase disparity.  Thus we can write the value of element $i$ for the knapsack problem as $v_i = \frac{1}{|A|}$ if $d_i \in A$ and $F^\text{opt}_i = 1$, $v_i = \frac{1}{|B|}$ if $d_i \in B$ and $F^\text{opt}_i = 0$, and $v_i = 0$ otherwise.

In Appendix~\ref{appendix:statdisp}, Algorithm \dn{xxx}, we present a $\mathcal{O}(N \log N)$ knapsack algorithm to find the classifier that minimizes PPR disparity over the Rashomon set $R_N(\epsilon)$. The key idea to make this algorithm efficient is that there are only two distinct values $v_i > 0$, $\frac{1}{|A|}$ and $\frac{1}{|B|}$ for group $A$ and $B$ respectively. Thus, the optimal knapsack solution will consist of the $k_A$ lowest-weight items from group $A$ and the $k_B$ lowest-weight items from group $B$, for some $k_A$ and $k_B$. We show in Appendix~\ref{appendix:statdisp} that $k_A$ and $k_B$ can be found in linear time through an incremental search (note that the naive approach of iterating over all possible $k_A$ and $k_B$ would require quadratic time), and thus the run time is dominated by the $\mathcal{O}(N\log N)$ sorting of items by weight.

\ignore{
Given the value and weight of each record, the algorithm calculates the final disparity and flip vector to decrease the disparity. Since $A$ and $B$ comprise elements of same magnitude, $\frac{1}{|A|}$ and $\frac{1}{|B|}$, respectively, the optimal solution will consist of $k_A$ items of lowest weight $A$ and $k_B$ items of lowest weight $B$, but we do not know $k_A$ and $k_B$. Initially, the algorithm calculates the maximum number of A elements, $k_A^\text{max}$, and B elements thereafter, $k_B^\text{max}$, that fit the capacity. Then, the maximum number of $B$ items that fit the capacity for each $k_A$ between 0 and $k_A^\text{max}$ is calculated and the minimum disparity is updated. 

By keeping track of $k_B$ items for a given $k_A$, one can incrementally update for $k_A-1$ by adding the lowest weight $B$ items not added until the capacity is full, resulting in a $O(N)$ algorithm. With $O(N ~\text{log} ~N)$ time to sort the weights to add the lowest weighted items, the overall time complexity is $O(N ~\text{log} ~N)$. Otherwise, searching through $B$ items separately for each $k_A$ leads to a naive quadratic-time $O(N^2)$ algorithm. 

 for Eq. \ref{sddefn} derivation, Eq. \ref{valsd} derivation, and algorithm to mitigate statistical disparity.
}

\subsubsection{Optimizing for error rate balance}
\label{sec:optimizing-TPR and FPR}

Given the notation above, in Appendix~\ref{appendix:errbal} we define the false positive rate disparity as: 
\begin{align*}
\text{disparity}_{FPR} = \left|\mathbf{E}[f(x_i) \:|\: d_i\in A, y_i = 0] - \mathbf{E}[f(x_i) \:|\: d_i \in B, y_i = 0] \right| = \left|\frac{(1-P_A) \cdot F_A}{||1-P_A||_1} - \frac{(1-P_B) \cdot F_B}{||1-P_B||_1}\right|,
\end{align*}
Assume wlog that subgroup $A$ has higher FPR, 
$\frac{(1-P_A) \cdot F_A}{||1-P_A||_1} > \frac{(1-P_B) \cdot F_B}{||1-P_B||_1}$. Then flipping a prediction in group $A$ from 1 to 0, or flipping a prediction in group $B$ from 0 to 1, reduces the disparity by $\frac{1-p_i}{||1-P_A||_1}$ or $\frac{1-p_i}{||1-P_B||_1}$ respectively, while other flips increase disparity.  Thus we can write the value of element $i$ for the knapsack problem as $v_i = \frac{1-p_i}{||1-P_A||_1}$ if $d_i \in A$ and $F^\text{opt}_i = 1$, $v_i = \frac{1-p_i}{||1-P_B||_1}$ if $d_i \in B$ and $F^\text{opt}_i = 0$, and $v_i = 0$ otherwise.

The derivation for true positive rate disparity, $\text{disparity}_{TPR} = \left|\mathbf{E}[f(x_i) \:|\: d_i\in A, y_i = 1] - \mathbf{E}[f(x_i) \:|\: d_i \in B, y_i = 1] \right|$, proceeds similarly (Appendix~\ref{appendix:errbal}), obtaining 
$v_i = \frac{p_i}{||P_A||_1}$ if $d_i \in A$ and $F^\text{opt}_i = 1$, $v_i = \frac{p_i}{||P_B||_1}$ if $d_i \in B$ and $F^\text{opt}_i = 0$, and $v_i = 0$ otherwise.

To minimize FPR or TPR disparity over the Rashomon set $R_N(\epsilon)$, we note that elements have more than two distinct values, so we cannot apply the solution for PPR above. Instead, as we describe in Appendix~\ref{appendix:errbal}, Algorithm \dn{xxx}, we approximate the 0-1 knapsack problem with the fractional knapsack problem: $\max \sum_i \theta_i v_i$ subject to $\theta_i \in [0,1]$ and $\sum_i \theta_i w_i \le N\epsilon$.
The standard solution to the fractional knapsack, which requires $\mathcal{O}(N\log N)$ time, adds elements to the knapsack ($\theta_i = 1$) in descending order of their ratio $\frac{v_i}{w_i}$ until no further elements can be (fully) added, then adds a fraction of the next element ($0 < \theta_i < 1$) to fill the remaining capacity. Rather than adding the fractional element, we show that it would reduce disparity by an amount $\theta_i v_i$
that is $\mathcal{O}(\frac{1}{N})$. Since the fractional knapsack solution $\sum \theta_i v_i$ is an upper bound on the 0-1 knapsack solution, 
we know that our solution (excluding the fractional element) reduces disparity to within $\mathcal{O}(\frac{1}{N})$ of the optimal disparity.

\subsection{Sampling models uniformly at random from the Rashomon set}
\label{sec:sampling}

The definition of the Rashomon set $R_N(\epsilon)$ in Section~\ref{sec:prelim} above suggests that a simple \emph{rejection sampling} approach could be used to draw models uniformly at random from the Rashomon set. That is, one can draw a binary flip vector $\theta \in \{0,1\}^N$ uniformly at random from the set of all $2^N$ possible flip vectors by drawing $\theta_i \sim \text{Bernoulli}(0.5)$ for all $i \in \{1 \ldots N\}$, and then keep only those vectors $\theta$ that are in the Rashomon set, i.e.,  with $\frac{\theta \cdot W_N}{N} \le \epsilon$.  The problem with this simple approach is that, as $N$ increases, the probability that $\theta$ is in the Rashomon set goes to 0.\footnote{This can be seen from Theorem~\ref{theorem:asymptotic_size_mainpaper} below: for $\epsilon$ less than half the average weight, $B(\epsilon) < 2$, and $\lim_{N \rightarrow \infty} \frac{|R_N(\epsilon)|}{2^N}$ = $\lim_{N \rightarrow \infty} \frac{B(\epsilon)^N}{2^N}$ = 0.} 

Thus we propose an alternative approach based on \emph{Gibbs sampling}~\cite{geman1984}. The key idea is to sequentially sample one element $\theta_i$ of the flip vector at a time, conditional on all the other elements $\theta_{-i}$.  While we do not have a closed form for the joint distribution of $\langle\theta_1,\ldots,\theta_N\rangle$ for $\theta \in R_N(\epsilon)$, computing the \emph{conditional} distribution of $\theta_i$ given $\theta_{-i}$ is straightforward. Let $\theta_{i=0} = \langle\theta_1,\ldots,\theta_{i-1},0,\theta_{i+1},\ldots,\theta_N\rangle$ and 
$\theta_{i=1} = \langle\theta_1,\ldots,\theta_{i-1},1,\theta_{i+1},\ldots,\theta_N\rangle$. Then we know that $\frac{\theta_{i=0}\cdot W_N}{N} \le 
\frac{\theta\cdot W_N}{N} \le
\frac{\theta_{i=1}\cdot W_N}{N}$. This implies that, if $\theta \in R_N(\epsilon)$ and $\theta_i = 1$, then $\theta_{i=0} $ and $\theta_{i=1}$ are both in the Rashomon set, so $\mbox{Pr}(\theta_i = 1 \:|\: \theta_{-i}) = \frac{1}{2}$. If $\theta \in R_N(\epsilon)$ and $\theta_i = 0$, then $\theta_{i=0} \in R_N(\epsilon)$, but we must check whether $\theta_{i=1} \in R_N(\epsilon)$, i.e., whether $\frac{\theta \cdot W_N + w_i}{N} \le \epsilon$. If so, then $\mbox{Pr}(\theta_i = 1 \:|\: \theta_{-i}) = \frac{1}{2}$, and if not, then 
$\mbox{Pr}(\theta_i = 1 \:|\: \theta_{-i}) = 0$.  Given this simple and computationally efficient conditional sampling step, our Gibbs sampling approach starts with the zero vector $\theta_0$, which is guaranteed to be in the Rashomon set, and iteratively samples $\theta_i \sim \text{Bernoulli}(p)$, where $p = \mbox{Pr}(\theta_i = 1 \:|\: \theta_{-i})$ as described above, for each $i \in \{1,\ldots,N\}$.  To ensure uncorrelated samples from the joint distribution, we take one sample every 10 iterations (where one iteration includes resampling all $N$ elements of $\theta$ in randomly permuted order), after an initial burn-in period of 500 iterations.  For each dataset and each value of $\epsilon$ considered, we run 10,000 iterations of Gibbs sampling, resulting in 950 samples.  Please see Appendix~\ref{appendix:gibbs}, Algorithm~\ref{algorithm:gibbs}, for the pseudocode of our Gibbs sampling algorithm.

\subsection{Baseline approach: sampling linear models from the Rashomon set}
\label{sec:linear}

As a simple baseline for comparison, which might be representative of how a company would typically choose a predictive model for deployment, we assume that a binary classifier is learned from a separate, large training dataset, where the model class is chosen $\emph{a priori}$ and therefore the set of possible flip vectors $\theta$ is restricted to members of that class. In particular, we assume that an $L_1$-penalized logistic regression model is learned; for consistency with the other methods in our experiments (since our evaluations use all $N$ data records), we use $k$-fold cross-validation and compute all metrics using predictions (for a given data record $d_i$) made using a model learned from the other $k-1$ folds (excluding the fold that contains $d_i$).  Moreover, since a company would typically explore the space of parameter values and choose a model with high accuracy, we learn penalized logistic regression models with different sources of random variation, evaluate their accuracy, and keep those models which are in the Rashomon set.

More precisely, to sample over the Rashomon set of $L_1$-penalized logistic regression models, for a given dataset and value of $\epsilon \in \{0.001, 0.002, \ldots, 0.02\}$, we sample 1,000 models, where for each model we randomly sample the number of cross-validation folds $k \in \{2, 3, \ldots, 10\}$, the logistic regression solver (lbfgs, liblinear, newton-cg, newton-cholesky, sag, or saga), and the amount of $L_1$ penalization $C\in \{ 0.001, 0.01, 0.1, 1.0, 10, 100 \}$ (note that lower values of $C$ correspond to more penalization), and then fit the penalized logistic regression model using scikit-learn.
Given the model's predictions $\langle f(x_1),\ldots,f(x_N)\rangle$, we compute the flip vector $\theta$, where $\theta_i = \mathbf{1}\{f(x_i) \ne f_\text{opt}(x_i) \}$, and include the sampled model in the Rashomon set if and only if $\frac{\theta \cdot W_N}{N} \le \epsilon$.

\subsection{Experiments on real data}
\label{sec:intentional-experiments}
%\paragraph{Experimental Methodology} 
Throughout this paper, we present experimental results on three real-world datasets that are commonly used as benchmarks in the fair machine learning literature: German Credit (``German''), Adult, and Heritage Health (``Health'').
Details of all three datasets are described in Appendix~\ref{appendix:datasets}.

As noted above, the Bayes-optimal probabilities $p_i$ are unknown for these real-world datasets, but can be well-estimated using sufficient training data.  Since we wish to compare the methods over all $N$ data records ($N=1,000$ for German, $N=46,443$ for Adult, and $N=184,308$ for Health) we performed 5-fold cross-validation to estimate these probabilities.  For each held-out 20\% of the data, we trained a model $\hat f_\text{opt}(x)$ using the remaining 80\% of the data to approximate the Bayes-optimal model $f_\text{opt}(x)$, and used its predicted probabilities $\hat p_i$ to estimate the Bayes-optimal probabilities $p_i$ for that fold.  More precisely, we trained logistic regression models on each dataset that matched typical (maximal) accuracies reported in the wider literature.  To check the robustness of our results to the choice of model used for estimation of $p_i$, we re-ran all experiments using the estimated probabilities $\hat p_i$ from XGBoost models learned using 5-fold cross-validation, as described in Appendix~\ref{appendix:robustness}, and found no substantial differences. 

To test the difference between randomly sampling from the Rashomon set and directly optimizing for the fairest model within the set on real data, for each dataset and each $\epsilon$ value, we compared the model found by optimizing the desired fairness metric (PPR, TPR, or FPR) over the Rashomon set $R_N(\epsilon)$, as described in Section~\ref{sec:optimizing-fairness}, to the distributions of models found by (i) uniform random sampling over all models (flip vectors) $\theta \in R_N(\epsilon)$, as described in Section~\ref{sec:sampling}, and (ii) sampling penalized logistic regression models (and corresponding flip vectors $\theta$) from $R_N(\epsilon)$, as described in Section~\ref{sec:linear}. 
For each distribution of samples, we report the mean and 95\% interquantile range, i.e., the 2.5 and 97.5 percentiles of the distribution.

We compare these approaches using three fairness criteria: statistical parity, or balanced positive prediction rate (PPR), balanced false positive rate (FPR), and balanced true positive rate (TPR).  
Disparities with respect to all three criteria were measured between the protected class ($A_i=a$) and non-protected class ($A_i\ne a$), using the sensitive attribute value for each dataset described in Appendix~\ref{appendix:datasets}. All three measures of disparity for a given flip vector $\theta$ were computed using the (estimated) Bayes-optimal probabilities $p_i$ and corresponding weights $w_i$, rather than the observed outcomes $y_i$, as described in Section~\ref{sec:optimizing-PPR} \dn{(CHECK THIS, OTHERWISE DESCRIBE HERE!)}  Results are shown in Figures~\ref{fig:PPR_disparity},~\ref{fig:FPR_disparity}, and~\ref{fig:TPR_disparity}. \dn{Describe results here? 
 Or just in takeaways?}

\ignore{Algorithms 1 (random sampling) 2, and 3 (optimal fairness) (available in Appendix \todo{APP}, using the estimated Bayes-optimal probabilities $\hat{p_i}$,Figure~\ref{fig:PPR_disparity} shows the average, and upper and lower 95 percentile range for models found with the optimal fairness search strategy, randomly sampling, and randomly sampling within linear models only.}

\subsection{Takeaways for policy and practice}
\label{sec:intentional-takeaways}
\begin{itemize}
    \item \textbf{A randomly sampled model within the Rashomon set is nowhere near as fair as the fairest model at any given $\epsilon$.} As we can see from in the gap between the blue and green lines in Figure~\ref{fig:PPR_disparity}, searching intentionally for the fairest model within the Rashomon set leads to much fairer models at the same $\epsilon$ than randomly sampling within the set. This shows us that a random model from the Rashomon set--- one selected on the basis of accuracy alone--- will have an extremely low chance of being the fairest, or even one of the fairer, models within the set. This in turn underscores the necessity of explicitly searching for fairer models before deployment-- i.e., an LDA search. 

    \item \textbf{In practice, it is often possible to completely eradicate disparities by searching within the Rashomon set for quite small $\epsilon$}. As we can see in Figure~\ref{fig:PPR_disparity}, for German Credit and Health datasets, a model exists that completely eradicates demographic disparity in the dataset for $\epsilon<0.005$, i.e. half a percentage point of accuracy loss. While the Adult dataset requires very slightly more than 2\% accuracy loss to fully eradicate the disparity, this is still a small enough gap considered to be acceptable based on case studies of LDA searches~\cite{colfax2022report3}.

    \item \textbf{Using repeated random sampling as a search strategy-- i.e., looking across many models selected on the basis of accuracy and searching for the fairest among them---can give mixed results.} While our theoretical setup does not map onto how LDA searches would be done in practice--- since we search through all the possible mappings of input to output for a dataset instead of generating actual parametric models---loosely, repeated random sampling corresponds to an LDA search that does not directly use protected attribute information until after all the models are trained, i.e., only as a step to evaluate models and choose among them post-hoc. Our optimal search method, on the other hand, corresponds to an LDA search method that uses some direct minimization of disparities across demographic groups during the model creation process, whether that be in hyperparameter tuning, optimization, or other parts of the pipeline. There is disagreement in the legal literature as to whether and to what extent interventions for disparity reduction across demographic group that use protected class information are legally permissible~\cite{ho2020affirmative, kim2022race, talia}. Our experimental results show that we gain a lot by being able to directly intervene using protected attributes---however, repeated random sampling without direct use of protected attributes can \dn{in some cases} be an effective technique as well, even if not as effective as direct intervention. In particular, we see that the German Credit results allow for a large reduction in disparity-- up to 57\% of the total the disparity reduced by $\epsilon=.015$ (1.5\% error tolerance from the optimal base model). \dn{Or is it 2\%? check this.} In addition, note that while random sampling over the \emph{entire} Rashomon set of all possible mappings of $x$ to $y$ is not particularly effective at reducing disparity in the Health dataset, only searching within linear models is in fact comparably quite effective--this is promising given that in practice, LDA searches can only be done within various model classes and not across all possible mappings. Divergence in the effectiveness of different random sampling methods based on model class is an interesting phenomenon that we look forward to studying in future work. 
\end{itemize}




%First, we experimentally demonstrate that while fair models exist within the Rashomon set, they can sometimes be difficult to find unless they are explicitly searched for. 

%we show that by combining algorithms 1 and 2, which search for random models within the Rashomon set and the fairest model within the Rashomon set respectively, 

